Surface fields and emergence of long-range couplings in classical uniaxial ferromagnetic arrays

Critical wetting is of crucial importance for the phase behaviour of a simple fluid or Ising magnet confined between walls that exert opposing surface fields so that one wall favours liquid (spin up), while the other favours gas (spin down). We show that arrays of boxes filled with fluid or Ising magnet and linked by channels with such ``opposing'' walls can exhibit long-range cooperative effects, on a length scale far exceeding the bulk correlation length. We give the theoretical foundations of these long-range couplings by using a lattice gas (Ising model) description of a system.

==> macros.tex <==
\usepackage[utf8]{inputenc}
\RequirePackage[switch,columnwise]{lineno}
%\usepackage{standalone}
\usepackage[T1]{fontenc}
\linespread{0.956}
\usepackage{lmodern}					% Version vectorielle de la police CM
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb,textcomp}
\usepackage[xcdraw]{xcolor}
\usepackage{colortbl}
\usepackage{tikz}
\usepackage{bm}
\usepackage{framed,xspace}
\usepackage{graphicx}
\usepackage{array,multirow}
%\usepackage[font=footnotesize,labelfont=bf]{caption}




\usepackage{natbib}
%\usepackage[backend=biber,natbib=true,sorting=none]{biblatex}
%\renewbibmacro{in:}{}
%\addbibresource{references.bib}
\usepackage[margin=2cm]{geometry}



\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{epsfig}
\usepackage{color}
\usepackage{psfrag}
\usepackage{epstopdf}
\usepackage{mathrsfs}
\usepackage{stmaryrd} % questa package genera la doppia parentesi quadra: \llbracket \rrbracket
\usepackage{empheq}
\usepackage{ifsym}
%\usepackage{showlabels}
\usepackage{bbding}
\usepackage{simpler-wick}

%\documentclass[notitlepage,reprint,amsmath,amssymb,aps]{revtex4-1}
%\usepackage{graphicx}% Include figure files
%\usepackage{dcolumn}% Align table columns on decimal point
%\usepackage{bm}% bold math
\usepackage{mathrsfs}

\usepackage{amsfonts}
%\usepackage{amssymb,textcomp}
%\usepackage[xcdraw]{xcolor}
%\usepackage{colortbl}
\usepackage{tikz}
%\usepackage{bm}
%\usepackage{framed,xspace}
\usepackage{graphicx}
%\usepackage{array,multirow}
\usepackage{tikz}
\usetikzlibrary{calc}
\usetikzlibrary{positioning}

%\usepackage{hyperref}

\interfootnotelinepenalty=10000

%\renewcommand{\figurename}{Fig.} % Rename Figure to Fig.

\newcommand{\fig}[1]{\parbox{2.0cm}{\epsfig{file=#1,height=1.1cm}}}




% Standard colors
\definecolor{cayenne}{RGB}{128, 0, 0}
\definecolor{1}{RGB}{98, 64, 27}
\definecolor{2}{RGB}{128,0,128}
\definecolor{3}{RGB}{0, 64, 120}
\definecolor{4}{RGB}{0, 88, 254}
\definecolor{5}{RGB}{0, 228, 64}
\definecolor{6}{RGB}{0, 128, 0}
\definecolor{moka}{RGB}{128, 64, 0}
\definecolor{orange}{RGB}{255, 128, 0}
\definecolor{azzurro1}{RGB}{30, 82, 255}
\definecolor{azzurro2}{RGB}{15, 127, 255}
\definecolor{blu1}{RGB}{0, 40, 128}
\definecolor{blu2}{RGB}{30, 88, 100}
% Apple colors
\definecolor{bluapple}{RGB}{0, 0, 255}
\definecolor{marroneapple}{RGB}{153, 102, 51}
\definecolor{cianoapple}{RGB}{0, 255, 255}
\definecolor{verdeapple}{RGB}{0, 255, 0}
\definecolor{magentaapple}{RGB}{255, 0, 255}
\definecolor{arancioapple}{RGB}{255, 128, 0}
\definecolor{violaapple}{RGB}{127, 0, 127}
\definecolor{rossoapple}{RGB}{255, 0, 0}
\definecolor{gialloapple}{RGB}{255, 255, 0}
\definecolor{aqua}{RGB}{0, 128, 255}
\definecolor{verde}{RGB}{1, 165, 1}

\newcommand{\com}[1]{\textcolor{red}{#1}}
\newcommand{\tdl}[1]{\textcolor{blue}{#1}}
\newcommand{\AS}[1]{\textcolor{orange}{AS: #1}}
\newcommand{\noteself}[1]{\textcolor{orange}{#1}}
\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}


\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{epsfig}
\usepackage{color}
\usepackage{psfrag}
\usepackage{epstopdf}
\usepackage{mathrsfs}
\usepackage{stmaryrd} % questa package genera la doppia parentesi quadra: \llbracket \rrbracket
\usepackage{empheq}
\usepackage{ifsym}
%\usepackage{showlabels}
\usepackage{bbding}
\usepackage{pifont}

\def\YES{ {\color{verde}{\ding{51}}} } %\checkmark
\def\NO{ {\color{red}{\ding{55}}} } %\XSolidBrush
\def\WIP{ \includegraphics[scale=0.95]{works.pdf} }

\usepackage[breakable, theorems, skins]{tcolorbox}
\tcbset{enhanced}

\DeclareRobustCommand{\mybox}[2][gray!20]{%
\begin{tcolorbox}[   %% Adjust the following parameters at will.
        breakable,
        left=0pt,
        right=0pt,
        top=0pt,
        bottom=0pt,
        colback=#1,
        colframe=#1,
        width=\dimexpr\columnwidth\relax, 
        enlarge left by=0mm,
        boxsep=5pt,
        arc=0pt,outer arc=0pt,
        ]
        #2
\end{tcolorbox}
}


\DeclareMathOperator*{\Mybigotimes}{\text{\raisebox{0.25ex}{\scalebox{0.7}{$\bigotimes$}}}}
  
%\newcomand{\NO}[1]{}



